Search for Double-Beta Decay of $\mathrm{^{130}Te}$ to the $0^+$ States of $\mathrm{^{130}Xe}$ with CUORE

The CUORE experiment is a large bolometric array searching for the lepton number violating neutrino-less double beta decay ($0\nu\beta\beta$) in the isotope $\mathrm{^{130}Te}$. In this work we present the latest results on two searches for the double beta decay (DBD) of $\mathrm{^{130}Te}$ to the first $0^{+}_2$ excited state of $\mathrm{^{130}Xe}$: the $0\nu\beta\beta$ decay and the Standard Model-allowed two-neutrinos double beta decay ($2\nu\beta\beta$). Both searches are based on a 372.5 kg$\times$yr TeO$_2$ exposure. The de-excitation gamma rays emitted by the excited Xe nucleus in the final state yield a unique signature, which can be searched for with low background by studying coincident events in two or more bolometers. The closely packed arrangement of the CUORE crystals constitutes a significant advantage in this regard. The median limit setting sensitivities at 90\% Credible Interval (C.I.) of the given searches were estimated as $\mathrm{S^{0\nu}_{1/2} = 5.6 \times 10^{24} \: \mathrm{yr}}$ for the ${0\nu\beta\beta}$ decay and $\mathrm{S^{2\nu}_{1/2} = 2.1 \times 10^{24} \: \mathrm{yr}}$ for the ${2\nu\beta\beta}$ decay. No significant evidence for either of the decay modes was observed and a Bayesian lower bound at $90\%$ C.I. on the decay half lives is obtained as: $\mathrm{(T_{1/2})^{0\nu}_{0^+_2} > 5.9 \times 10^{24} \: \mathrm{yr}}$ for the $0\nu\beta\beta$ mode and $\mathrm{(T_{1/2})^{2\nu}_{0^+_2} > 1.3 \times 10^{24} \: \mathrm{yr}}$ for the $2\nu\beta\beta$ mode. These represent the most stringent limits on the DBD of $^{130}$Te to excited states and improve by a factor $\sim5$ the previous results on this process.

==> Makefile <==
# input
MAIN					= main

MAIN_TEX				= ${MAIN}.tex
MAIN_PDF				= ${MAIN}.pdf

BIBLIOGRAPHY		= ref.bib

# clean
FILE_CLEAN			= *.aux *.bbl *.blg *.brf *.idx *.ilg *.ind *.log *.out *~ *Notes.bib
FILE_DISTCLEAN		= ${MAIN_PDF} ${OUTPUT_PDF}

.PHONY:	pdf biblio \
			rename \
			distclean clean

pdf:	${MAIN_TEX}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
biblio: ${MAIN_TEX} ${BIBLIOGRAPHY} 
	pdflatex ${MAIN}
	bibtex ${MAIN}
#	makeindex ${MAIN}
	pdflatex ${MAIN}
	pdflatex ${MAIN}
	evince ${MAIN_PDF}
	
view:	${MAIN_PDF}
	evince ${MAIN_PDF}
	
distclean:	clean
	rm -f ${FILE_DISTCLEAN}

clean:
	rm -f ${FILE_CLEAN}

